Human-In-the-Loop Software Development Agents

Recently, Large Language Models (LLMs)-based multi-agent paradigms for software engineering are introduced to automatically resolve software development tasks (e.g., from a given issue to source code). However, existing work is evaluated based on historical benchmark datasets, rarely considers human feedback at each stage of the automated software development process, and has not been deployed in practice. In this paper, we introduce a Human-in-the-loop LLM-based Agents framework (HULA) for software development that allows software engineers to refine and guide LLMs when generating coding plans and source code for a given task. We design, implement, and deploy the HULA framework into Atlassian JIRA for internal uses. Through a multi-stage evaluation of the HULA framework, Atlassian software engineers perceive that HULA can minimize the overall development time and effort, especially in initiating a coding plan and writing code for straightforward tasks. On the other hand, challenges around code quality remain a concern in some cases. We draw lessons learned and discuss opportunities for future work, which will pave the way for the advancement of LLM-based agents in software development.

==> sections/4.1_evaluation_old.tex <==




\subsection{Evaluation Data Curation}
In order to evaluate the performance of \ours, a dataset of software development tasks with sufficient information documented and human-written code is required.
For each task, the documented information is needed to provide sufficient context for \ours~to generate code on, and the human-written code is needed for \ours~to evaluate against.
In this section, we describe 2 evaluation datasets chosen for \ours~evaluation, i.e., SWE-bench and our internal dataset, along with our methodological justifications.

\textbf{SWE-bench.} Jimenez~\ea~\cite{jimenez2023swe} proposed \emph{SWE-bench}, a benchmark of 2,294 software engineering issues and corresponding pull requests (PRs) sourced from real 12 open-source Python repositories on GitHub.
The issue's context includes bug reports, code refactoring suggestions, code optimizations, feature requests, etc.
% <<NEED TO ADD WHAT THE TASKS ARE ABOUT (e.g., FAILING UNIT TEST). ALSO NEED TO MENTION THIS SET IS USING UNIT TEST FOR FUNCTIONALITY CORRECTNESS AS THE BENCHMARK, WHICH IS IT's STRENGTH (SAY WE WILL EXPLAIN THIS IN THE NEXT SECTION>>
Given the code repository and issue documented information, the benchmark aims to evaluate the ability of a software development agent to resolve issues, using unit tests as a success measurement.
SWE-bench becomes a new challenging test-bed for the software development agents. 
% with the top score of 20\% resolved rate on the full test set.\footnote{https://www.swebench.com}
Therefore, we include the SWE-bench dataset in our evaluation to compare our software development agent with the research community. 
In this evaluation, we use a subset of the original test set from SWE-bench that is verified to be non-problematic by human annotators: SWE-bench Verified~\cite{sweverify2024}.

\textit{Limitations:} 
Nonetheless, to sufficiently gauge our software development agent performance for production use, we need diverse contexts of software development tasks.
% While SWE-bench can evaluate the software development agent to some extend, the diversity of the benchmark is restricted with 3 limitations: 1) the benchmark is solely based on Python programming language, 2) the benchmark is solely based on open source projects that may not reflect our target industrial settings
While SWE-bench offers a useful framework for evaluating software development agents, it has three key limitations: 
(1) the scope is confined to issues in the Python programming language, 
(2) the dataset is derived solely from open-source projects, which may not fully represent the complexities of enterprise proprietary software development, 
and (3) the benchmark yields only binary results (i.e., whether the generated code passes or fails a test case) without providing how closely the generated code is to the intended solution.
These limitations led us to build our internal dataset that consists of diverse programming languages and contexts.

\textbf{Internal Dataset.} We curated our internal dataset from our software development data, containing software development tasks from JIRA Software (i.e., a task management system) and human-written code from Bitbucket (i.e., Git-based source code repository).
This dataset represents the proprietary industrial software development, which captures diverse contexts of development tasks, programming languages, software repositories, and development teams.
% As the goal of our software development agent is to assist in the real-world industrial settings, our Atlassian large production-grade codebase that contains varying products with various programming languages and tasks should be suitable for our evaluation.

We randomly sampled issues from our JIRA Software and the corresponding pull requests (PRs) from BitBucket.
To be able to examine the performance of \ours~against different task complexities, we sampled our dataset based on Story Points (i.e., a unit representing the relative complexity of a development task estimated by the software development team~\cite{cohn2005agile}).
We first scoped our dataset to the difficulty level of one Story Point to examine how well \ours~can solve a relatively low complexity task.
One sample data is a triplet of $\langle$documented information in JIRA issue, codebase url, and PR$\rangle$.
The documented information of an issue consists of a short summary and a description that describe more detail.
Generally, the issue description contains necessary documented information for human to understand the work to be done, e.g., a user story, definition of done, acceptance criteria, or code examples~\cite{pasuksmit2021towards}.
In our dataset, the issue summary has a median length of 52.5 characters, while the issue descriptions have a median length of 251.0 characters.
Table~\ref{tab:internal_stat} shows the statistical summary of issue information (i.e., topics and descriptions, respectively).
The PR information is in a format of a \emph{code diff} representing the chuck of codebase edited by human to resolve the issue task.
¢

In total, our internal dataset contains 368 JIRA issues from 94 software repositories; thus, the median of 3 issue per repository.
The issues' context ranges from front-end developments, back-end developments, data analytics, security patches, product migrations, configuration updates, bug fixes, and more.
The PRs solutions contain 24 types of file extensions with more than 10 programming languages including TypeScript, Java, Kotlin, Go, Python, Scala, etc. 
Figure~\ref{tab:prog_lang} show the top 10 most frequency file types in the internal dataset.

\subsection{Evaluation Framework}
Evaluating the software development agents is challenging due to various factors including the intricate nature of software engineering tasks and the complexity in designing effective metrics.
% Our primary objective is to create a software development agent that seamlessly assists software engineers in coding and enhances their productivity.
To achieve this, we meticulously designed our evaluation framework to assess performance through multiple dimensions: ``offline evaluation'' based on benchmark datasets, ``online evaluation'' based on users interactions and events-based data, and ``user feedback'' based on surveys with internal software engineers.

% The definition of good code quality for an AutoDev-generated code? → human-written code comparison and impact on software development
% What approach should we use to track if AutoDev-generated code is of similar quality to human-written code?
% What metrics should be used to track the impact of AutoDev on the software development process?



\subsubsection{Online Evaluation} involves assessing our software development agent performance in real-world production settings (i.e., JIRA) where user interact with the application in real-time.
This evaluation allows us to capture insights from actual usage conditions where user behavior are involve.
In this online evaluation, we select four evaluation metrics as follows:

\begin{itemize}
    \item \textbf{Issue Generated Code Rate} measure the number of issue generated code with the software development agent to the total number of issue with user interact with the software development agent.
    %  Issues generated code / Issues AutoDev button clicked
    
    \item \textbf{Issue Resolved Rate} measure the number of issues resolved with the software development agent generated PRs to the total number of issue with user interact with the software development agent.
    % Issues with merged AutoDev PR / Issues that clicked AutoDev

    \item \textbf{Generated-PR Merged Rate} measure the number of the software development agent generated PRs that merged into production to the total number of the software development agent generated code.
    % PRs merged with code generated by AutoDev / Total PRs raised with code generated by AutoDev

    \item \textbf{Issue Usage Funnel} use to monitor the usage data from users interaction on the triggered \ours~issues.
\end{itemize}

\subsection{Internal Deployment}
% dogfooding -- participant program
% # participants
As Atlassian is a large company and \ours~is still in the early development stages, we must deploy our new agent cautiously.
We divide the internal deployment into two phases: the internal alpha deployment and the internal general deployment.
This approach allows users to gradually adapt to the new experience while enabling us to gather and understand their feedback effectively.

\textbf{The internal alpha deployment.} 
In June 2024, we deploy \ours~to a very small number of users called an alpha group.
This alpha group comprises two teams of software engineers working on different products, totaling 45 engineers.
We let the alpha users use \ours~for 2 weeks to monitor the usage, performance, and reliability.
Furthermore, we conduct the in-depth usability interviews with 8 engineers from the alpha group to gain deeper insights into user experiences and the quality of the generated code.
At the conclusion of this internal alpha deployment, we iteratively redesign and improve the \ours~agent based on the feedback received.

\textbf{The internal general deployment.}
After several iterations to stabilize the design of our \ours~workflow, we expand the deployment to broader Atlassian teams. 
Beginning with 260 engineers in early July 2024, we gradually rolled out the agent to software engineers, prioritizing projects and story point issue estimations.
Since our offline evaluation tested the \ours~agent on an internal dataset of 1-story point issues, we initially limited the general deployment to issues marked as 1-story point. 
% By the end of August 2024, we had successfully extended coverage to over 1,600 engineers and 15,000 eligible issues, with 40\% being 1-story point issues.
By mid-September 2024, we successfully scale to cover over 2,600 engineers and 22,000 eligible issues, with 20\% being 1-story point issues.

It is important to note that the full expansion commenced at the beginning of September; hence, the usage data reported in this paper may be delayed and not directly comparable to the total number of eligible engineers and issues.

\subsection{User Feedback}
\textcolor{blue}{moved from user perception}
\ours~aims to assist software engineers in JIRA platform; therefore, the engineers' perceptions on \ours~are crucial.
During the internal deployment, we collect user feedback in free-form texts from JIRA in-platform feedback channel and follow-up questions via Slack communications.
In total, we gather feedback from 32 software engineers who use \ours~to generate code at least once.
We perform open coding to extract category of the qualitative feedback, then, perform three iterations of card sorting to categorize feedback into three main themes: why the generated PRs are merged (Figure~\ref{fig:autodev-merged}), why the generated PRs are not merged (Figure~\ref{fig:autodev-not-merge}), and what are the areas of improvement (Figure~\ref{fig:autodev-improve}).


==> sections/4.2_findings_old.tex <==


\textbf{\ours~file matched Recall and Perfect F1 are significantly decline in the internal dataset compare to the SWE-bench dataset.}
This is due to the differences in input detail and the number of changed files between the two datasets.
In the SWE-bench Verified dataset, issue descriptions have a median length of 1,185 characters, often including code snippets and file names that need to be changed. 
Conversely, in the internal dataset, the combined median length of the issue topic and description is just over 300 characters, making it three times shorter than that of SWE-bench. 
Additionally, the SWE-bench dataset contains fewer reference changed files, averaging 2.2 per issue, compared to 3.5 in our internal dataset.
These factors significantly impact the ability to identify the files to be changed, leading to a decline in the accuracy of file matching results in the internal dataset.


\textbf{\ours~achieve 29.9\% code similarity to human-written code on the internal dataset, which is 14.8\% lower than the 44.7\% similarity observed on SWE-bench.}
Given the lower file matching results, it is anticipated that the similarity between \ours-generated code and the reference code would also be reduced.
This does not imply that \ours~underperforms; in fact, the model achieves a 31.4\% issue resolved rate (unit test passed) on the SWE-bench, demonstrating a well performance to some extend on the SWE-bench leaderboard.
Therefore, the results highlights the complexities and challenges presented in our internal dataset.
These complexities include the diversity of programming languages and the variety of software engineering tasks between the two datasets. 
The SWE-bench dataset consists solely of Python source code, whereas the internal dataset includes over 10 programming languages and over 20 file type extensions.
Furthermore, different to the SWE-bench dataset, which includes 12 open-source repositories, the internal dataset comprises a variety of 94 production repositories. 
These challenging factors could strengthen the robustness in the evaluation process; however, lessen the evaluation results.
% Lastly, despite the challenging of the internal dataset, \ours~still generates code with 29.9\% similar to the human-written code. 

% \textbf{RQ2.} How well does AutoDev perform in practice?



% based on the user feedback analysis, while the lessons learned will be discussed in the next section (Section~\ref{sec:future}).

\textbf{\ours~drives an interesting experience in JIRA while helping with the initial coding process.}
Introducing a coding agent into JIRA task management platform gives a new and interesting experience, highlighted by two engineers.
While four engineers report that plans generated by \ours~are reasonably correct to proceed to the code generation step, some of them mention that it also help them improve the code structure.
In addition, three engineers reported \ours~aid them in the initial coding process, such as scaffolding code. 

\textbf{\ours~performs better on issues with a simple logic, small changes, and fewer changed files.}
While ten engineers report that \ours~successfully solves their tasks, four engineers suggest the tasks given to \ours~should be simple unless the changes might be incomplete.
This observation aligns with the quantitative results in our offline evaluation, where \ours~shows better performance on the dataset with fewer changed files, such as SWE-bench, compare to our internal dataset.

\textbf{Important factors influencing the decision to merge generated PRs are code functionality and changes completeness.}
In feedback regarding failed PR merges, engineers frequently highlight difficulties related to incomplete code changes.
Many engineers noted that while \ours~can partially address tasks, it often fails to implement all the necessary changes.
This shortcoming often results in the generated code being discarded, prompting engineers to revert to writing the code themselves.
This observation aligns with the issue usage funnel in our online evaluation, where there is a notable drop-off between the code generation stage and the PR raised stage.
These factors will be discussed in detail in the next section, focusing on the lessons learned and the potential future directions for the community.

==> sections/5_related_works.tex <==
\section{Related works}\label{sec:related}
In this section, we discuss the evolution of code generation benchmarks and LLM-based software development agents.

\subsection{Code Generation Benchmark}
% LLMs agent test on open source data
Code generation has been a prominent research topic for decades, with numerous studies proposing benchmark datasets~\cite{jimenez2023swe, lu2021codexglue, austin2021mbpp, hendrycks2021apps, chen2021humaneval, yan2023codescope}.
Lu~\ea~\cite{lu2021codexglue} propose CodeXGLUE, a benchmark dataset and open challenge for code intelligence which includes 14 datasets for 10 code intelligence tasks (i.e., code-code~\cite{allamanis2013mining, raychev2016probabilistic}, code-text~\cite{iyer2018mapping, husain2019codesearchnet}, text-code~\cite{husain2019codesearchnet}, text-text~\cite{lu2021codexglue}).
However, the datasets mostly evaluate results based on semantics (i.e., textual-based) which is not the objective of code.
To address this limitation, HumanEval~\cite{chen2021humaneval}, MBPP~\cite{austin2021mbpp} and APPS~\cite{hendrycks2021apps} datasets are introduced with the test cases to evaluate the code functionality of the generated code.
However, these datasets involve source code only at the file level.
To address this limitation, Jimenez~\ea~\cite{jimenez2023swe} propose SWE-Bench, a dataset for addressing issues at the repository level with unit test evaluation.
However, SWE-bench can be costly and contains particularly difficult or problematic tasks~\cite{xia2024agentless}.
As a result, researchers have focused on manually identifying high-quality tasks that feature a reasonable level of difficulty issues, well-defined descriptions, and adequate evaluation tests. 
This effort has led to the creation of SWE-bench Verified~\cite{sweverify2024}, which is used as a part of the offline evaluation setting in this paper.

% a human annotation campaign with professional software developers to screen each sample of the SWE-bench test set for appropriately scoped unit tests and well-specified issue descriptions.

% benchmark dataset and open challenge for code intelligence. It includes a collection of code intelligence tasks and a platform for model evaluation and comparison. CodeXGLUE stands for General Language Understanding Evaluation benchmark for CODE. It includes 14 datasets for 10 diversified code intelligence tasks covering the following scenarios:

% On HumanEval, a new evaluation set we release to measure functional correctness for synthesizing programs from docstrings

% The benchmark consists of around 1,000 crowd-sourced Python programming problems, designed to be solvable by entry level programmers, covering programming fundamentals, standard library functionality, and so on. Each problem consists of a task description, code solution and 3 automated test cases.

% APPS is a benchmark for code generation with 10000 problems. It can be used to evaluate the ability of language models to generate code from natural language specifications. 

% Yet, the findings, in general, are limited to the research environments with specific open source projects scope~\cite{hou2023large} and programming languages.

% \subsection{Code Evaluation Metric}
% Previous research proposing code evaluation metrics~\cite{papineni2002bleu, lin2004rouge, zhou2023codebertscore, ren2020codebleu}

\subsection{LLM-based Software Development Agent}
% LLM-based agent has been popularly applied to automate throughout the software engineering tasks.
% From the software development~\cite{}, program repair~\cite{}, software testing~\cite{}, to the end-to-end software engineering process~\cite{}.
Since the introduction of SWE-bench~\cite{jimenez2023swe}, the intricate challenge of addressing software issues at the repository level has attracted significant attention from both academia and industry. 
Numerous studies have proposed frameworks~\cite{yang2024swe, zhang2024autocoderover, chen2024coder, tao2024magis, xia2024agentless, arora2024masai, ma2024understand} aim to tackle these complex problems.
For example, Yang~\ea~\cite{yang2024swe} propose SWE-agent, an LLM-based agent that is built on top of a Linux shell, enabling the agent to effectively search, navigate, edit, and execute code commands.
Zhange~\ea~\cite{zhang2024autocoderover} propose AutoCodeRover, an LLM-based agent with code search on AST (i.e., Abstract Syntax Tree) and spectrum-based fault localization using test-suite.
Ma~\ea~\cite{ma2024understand} propose RepoUnderstander, an LLM-based agent with a Monte Carlo tree search-based exploration strategy on the repository knowledge graph.
Tao~\ea~\cite{tao2024magis} propose Magis, a multi-agent framework with four customized roles: manager, repository custodian, developer, and quality assurance engineer.
Chen~\ea~\cite{chen2024coder} propose CodeR, a multi-agent framework with pre-defined task graphs.
Arora~\ea~\cite{arora2024masai} propose Masai, a modular framework that divides the problem into multiple sub-problems for LLM-based agents.
Xia~\ea~\cite{xia2024agentless} propose Agentless, an agentless approach with simplistic two processes of localization and repair, without other complex tools.

Different to the existing works, our paper focuses on studying an LLM-based software development agent in practicality.


%%% REF %%%%
% To attempt to answer this question, we build AGENTLESS – an agentless approach to automatically solve software devel- opment problems. Compared to the verbose and complex setup of agent- based approaches, AGENTLESS employs a simplistic two-phase process of localization followed by repair, without letting the LLM decide future ac- tions or operate with complex tools

% we propose a Modular Architecture for Software-engineering AI (MASAI) agents, where different LLM-powered sub-agents are instantiated with well-defined objectives and strategies tuned to achieve those objectives.
% Our modular architecture offers several advantages: (1) employing and tuning different problem-solving strategies across sub-agents, (2) enabling sub-agents to gather information from different sources scattered throughout a repository, and (3) avoiding unnecessarily long trajectories which inflate costs and add extraneous context. 

% LLM-based Multi- Agent framework for GitHub Issue reSolution, MAGIS, consisting of four agents customized for software evolution: Manager, Repository Custodian, Developer, and Quality Assurance Engineer agents. This framework leverages the collaboration of various agents in the planning and coding process to unlock the potential of LLMs to resolve GitHub issues.











% [Codebase → Issue → Development → Pull request → Integration]
% -An issue ticket is raised in JIRA (An example of issue summary and issue description)
% -Johny starts working on an issue by creating a new branch in BitBucket repository and developing a feature in the codebase.
% -Johny finishes the development and raises a pull request in the BitBucket repository.
% -The PR is merged back into the main branch codebase.
% -The JIRA issue ticket is marked as done and resolved.

% -Pick up a ticket
% -Plan how to approach it
% -Write code and raise PR
% -Review PR, accept changes and merge

% \subsection{The Motivation: a pre-Autodev survey}

==> sections/table_improvement.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{The Area of Improvement from User Feedback (n=72).}
\label{tab:area_improvement}
\begin{tabular}{p{2cm}|p{3cm}|l|l}
\textbf{Theme} & \textbf{Sub-theme} & \textbf{Topic} & \textbf{Detail} \\
\hline

\multirow{9}{*}{Input \& Context} & \multirow{4}{*}{\shortstack[l]{Context enhancement \\(n=11)} } & Documents & \begin{tabular}[c]{@{}l@{}}Type definition\\ Libraries documents\\ Name conventions\end{tabular} \\
  \cline{3-4}
  
 &  & Practices & \begin{tabular}[c]{@{}l@{}}Design pattern\\ Best coding practices\end{tabular} \\
   \cline{3-4}
   
 &  & Repository data & \begin{tabular}[c]{@{}l@{}}Issue and repository dependencies\\ Historical commits\\ README files\\ Previous solution to similar task\end{tabular} \\
   \cline{3-4}
   
 &  & Tools & \begin{tabular}[c]{@{}l@{}}CI status\\ Atlassian's packages and tools\end{tabular} \\
 \cline{2-4}
 
 & \multirow{2}{*}{Input guidance (n=9)} & Information & \begin{tabular}[c]{@{}l@{}}Good input description\\ How to use properly\end{tabular} \\
  \cline{3-4}
  
 &  & Examples & \begin{tabular}[c]{@{}l@{}}Appropriate issues\\ Templates for different kind of tasks\end{tabular} \\
 \cline{2-4}
 
 & \multirow{3}{*}{\shortstack[l]{Context personalized \\ options (n=4)}} & Input & Customize code validation tools for repository \\
  \cline{3-4}
  
 &  & Process & \begin{tabular}[c]{@{}l@{}}External services\\ Dashboard editable components\end{tabular} \\
  \cline{3-4}
 &  & Output & Git branches \\
 \hline
 
\multirow{4}{*}{\shortstack[l]{Planing \&\\ Coding process}} & Improve plan detail (n=3) & Plan & More refined planning steps \\
 \cline{2-4}
 
 & Time-efficiency (n=6) & Process & Optimize background process \\
  \cline{2-4}
  
 & \shortstack[l]{Enhance code validation \\ (n=7)} & Integrate code validation tools & \begin{tabular}[c]{@{}l@{}}Coding style conventions\\ Linters\\ Compilers\\ CI/CD builds\\ Non-functionality requirements\end{tabular} \\
  \cline{2-4}
  
 & \shortstack[l]{Code functionality \& \\completeness (n=16)} & Performance & Improve based-model \\
 \hline
 
\multirow{5}{*}{\shortstack[l]{Scope \& \\Workflow}} & \multirow{2}{*}{\shortstack[l]{Expand issue scope \\(n=5)} } & Tasks & \begin{tabular}[c]{@{}l@{}}Larger task\\ More complex task\end{tabular} \\
 \cline{3-4}
 &  & Characteristics & \begin{tabular}[c]{@{}l@{}}More programming languages and libraries\\ Multi-repositories (e.g., issue and code dependencies)\\
 Multi-modal input (e.g., image and video) \end{tabular} \\
  \cline{2-4}
  
 & \multirow{2}{*}{\shortstack[l]{Improve UXUI workflow \\(n=17)} } & Interface & \begin{tabular}[c]{@{}l@{}}Improve feature feedback\\ Warning when model’s unconfident\\ More input options\end{tabular} \\
  \cline{3-4}
  
 &  & Workflow & \begin{tabular}[c]{@{}l@{}}Improve altering/revisiting workflow\\ Integrate with IDE\end{tabular} \\
  \cline{2-4}
  
 & \shortstack[l]{Multi-task automation\\ (n=5)} & More complete automation & \begin{tabular}[c]{@{}l@{}}Corresponding test case generation\\ Task decomposition\\ PR description generation\end{tabular}
\end{tabular}
\end{table*}

